Local Collaborative Autoencoders

Top-N recommendation is a challenging problem because complex and sparse user-item interactions should be adequately addressed to achieve high-quality recommendation results. The local latent factor approach has been successfully used with multiple local models to capture diverse user preferences with different sub-communities. However, previous studies have not fully explored the potential of local models, and failed to identify many small and coherent sub-communities. In this paper, we present Local Collaborative Autoencoders (LOCA), a generalized local latent factor framework. Specifically, LOCA adopts different neighborhood ranges at the training and inference stages. Besides, LOCA uses a novel sub-community discovery method, maximizing the coverage of a union of local models and employing a large number of diverse local models. By adopting autoencoders as the base model, LOCA captures latent non-linear patterns representing meaningful user-item interactions within sub-communities. Our experimental results demonstrate that LOCA is scalable and outperforms state-of-the-art models on several public benchmarks, by 2.99~4.70% in Recall and 1.02~7.95% in NDCG, respectively.

==> Code_training.tex <==
\SetKwInOut{Parameter}{Parameters}

\begin{algorithm}[h]
  \KwIn{The number of local models $q$, two kernel bandwidths $h_W$ and $h_T$, regularization $\lambda$}

  Choose $q$ anchors using coverage-based selection in Sec.~\ref{sec:anchor}.
  
  \For {$j = 1, ..., q$ \textbf{\textrm{parallel}}}
  {
    Calculate $\mathbf{t}^{(j)}$ for training the local model using Eq.~(\ref{eq:train_kernel}).
    
    Calculate $\mathbf{w}^{(j)}$ for inferring the local model using Eq.~(\ref{eq:aggregate_kernel}).
    
    Train $M^{\text{local}}(\mathbf{R}^{(j)};\theta^{(j)})$ using Eq.~(\ref{eq:train_local}).
  }
  
  Train $M^{\text{global}}(\mathbf{R};\theta^{(g)})$ using Eq.~(\ref{eq:train_global}).

  Predict $\hat{\mathbf{R}}$ using Eq.~(\ref{eq:global_local_aggregation}).
  
\caption{Training and inference procedure for COLA}\label{alg:training}
\end{algorithm}


==> backup/Fig789_ablation.tex <==
% 5.5 Ablation Study for Hyperparameters

\begin{figure*}[t]
\centering
\begin{tabular}{ccc}
\includegraphics[width=0.29\textwidth]{Figures/Fig7_train_h_1m.pdf} &
\includegraphics[width=0.29\textwidth]{Figures/Fig7_train_h_10m.pdf} &
\includegraphics[width=0.29\textwidth]{Figures/Fig7_train_h_amusic.pdf} \\
(a) ML1M & (b) ML10M & (c) AMusic \\
\end{tabular}
\caption{NDCG@100 vs. kernel bandwidth $h_T$ in learning local models. ($h_W=0.4$)}\label{fig:train_h}
\end{figure*}

\begin{figure*}[t]
\centering
\begin{tabular}{ccc}
\includegraphics[width=0.29\textwidth]{Figures/Fig8_test_h_1m.pdf} &
\includegraphics[width=0.29\textwidth]{Figures/Fig8_test_h_10m.pdf} &
\includegraphics[width=0.29\textwidth]{Figures/Fig8_test_h_amusic.pdf} \\
(a) ML1M & (b) ML10M & (c) AMusic \\
\end{tabular}
\caption{NDCG@100 vs. kernel bandwidth $h_W$ in aggregating local models. ($h_T=1.0$)}
\label{fig:aggregate_h}
\end{figure*}

\iffalse
\begin{figure*}[t!]
\centering
\begin{tabular}{ccc}
\includegraphics[width=0.29\textwidth]{Figures/Fig9_dimension_100k.pdf} &
\includegraphics[width=0.29\textwidth]{Figures/Fig9_dimension_1m.pdf} &
\includegraphics[width=0.29\textwidth]{Figures/Fig9_dimension_am.pdf} \\
(a) ML-100K & (b) ML-1M & (c) AMusic \\
\end{tabular}
\caption{NDCG@100 vs. the size $k$ of embedding dimensions in local models.}\label{fig:dimension}
\end{figure*}
\fi
